CLIC e+e- Linear Collider Studies - Input to the Snowmass process 2013

This paper addresses the issues in question for Energy Frontier Lepton and Gamma Colliders by the Frontier Capabilities group of the Snowmass 2013 process and is structured accordingly. It will be accompanied by a paper describing the Detector and Physics studies for the CLIC project currently in preparation for submission to the Energy Frontier group.

==> globalrevision.tex <==
\SetWatermarkText{Draft Revision exported}
\newcommand{\buildtimestamp}{}
\newcommand{\buildrevision}{exported}

